Semantic Variation in Online Communities of Practice

We introduce a framework for quantifying semantic variation of common words in Communities of Practice and in sets of topic-related communities. We show that while some meaning shifts are shared across related communities, others are community-specific, and therefore independent from the discussed topic. We propose such findings as evidence in favour of sociolinguistic theories of socially-driven semantic variation. Results are evaluated using an independent language modelling task. Furthermore, we investigate extralinguistic features and show that factors such as prominence and dissemination of words are related to semantic variation.

==> discussion.tex <==

 


%\raq{about less Diss for community shift words, I think this means that since the domain-related communities share quite a few members, if the shift was very disseminated it would spread to the domain and thus be a domain shift. A community-specific shift presumably can only happen if it takes place among users who are relatively `isolated'. Of course we cannot test whether the words are only disseminated among the users who are not members of other communities in the domain, but could be a line for future work.}



==> factors-old.tex <==
Having confirmed that the semantic shift indices proposed in Section~\ref{sec:measures} capture  variation that is noticeable in an external language modelling task, we now turn to analysing the factors that may be related to the presence of such variation.  

\subsection{Features}
\label{sec:factors-features}

We consider four features capturing different properties of word {\em forms} and investigate their effect on meaning variation:

% all features in the range [0,1] ?

\paragraph{Frequency.} 
It is known that more frequent words have a tendency to be more polysemous \cite{Zipf49}, are more semantically stable over time \cite{hamilton2016diachronic}, and evolve at slower rates across languages \cite{pagel2007frequency}. Word frequency may therefore play a role in semantic variation across communities of practice. We compute word frequency as the log-scaled relative frequency of a word in a given community: 
\begin{eqnarray*}
{\rm Freq}(w,c) & = &  \log_{10}(N^w_c / N_c)
\end{eqnarray*}
where $N_c$ is the total number of words in the sample dataset of community $c$ and $N^w_c$ the number of occurrences of word $w$ in that sample.

\paragraph{Prominence.} 
Many measures have been proposed to weight the prominence of a word in a language sample, including TF-IDF. Our choice here is inspired by literature on terminology extraction \cite{velardi2007termextractor}. We compute the prominence of $w$ as its frequency in a domain ($N^w_D$) relative to its frequency in general language use ($N^w_g$) or as its frequency in a community ($N^w_c$) relative to its frequency in a  domain:
\begin{eqnarray*}
{\rm Pro}(w,D) & = & N^w_D / (N^w_D + N^w_g)\\
{\rm Pro}(w,c) & = & N^w_c / (N^w_c + N^w_{D\setminus\{c\}})
\end{eqnarray*}
Community-specific jargon or slang words will typically have very high prominence. In contrast, we hypothesise that common words exhibiting semantic variation as a result of community conventions --- which are our focus here --- are likely to {\em not} be singled out by very high  prominence values.  Nevertheless, their level of prominence may still be a determiner of variation. 


%Given our hypothesis that semantic variation is not restricted to jargon (technical terms) but may affect common words as a result of the dynamics of interaction, we expect to find words that undergo a semantic shift even if they do not exhibit high prominence values. 

%\raq{This is indeed related to the issue of common words vs technical words/jargon. We will need to refine this as we make this aspect clearer in earlier sections of the paper.}
%\mdt{I have added parts related to this in 4.2 and 5. I think that the way you state out hypothesis here is fine}
%MARCO: As you said several times, frequency and relevance are related, so probably the hypotheses for the two of them will be the same. I don't have a clear idea now: probably, since we want to consider common words, exactly the fact they have similar DR and freq in general lanaguage and domain/community make them 'common', and therefore I don't expect domain and common shift to go up as freq and dr go up. Yes, now that I think about it, I think that exactly these two features can be the solution for identifying 'common words'. Let me know what you think.


\paragraph{Specificity.} 
Besides frequency-related aspects, we also want to capture the extent to which a given word $w$ appears in a restricted set of contexts. We approximate this by computing the collocational score of every bigram containing $w$ and then scoring them using log-likelihood ratio as association measure \cite{dunning1993accurate,manning1999foundations}.\footnote{We used the NLTK implementation \url{http://www.nltk.org/howto/collocations.html}} We take the value of the highest ranked bigram as a proxy for the contextual specificity ${\rm Spe}(w,c)$ of $w$ in community $c$. The feature values are normalised per community to obtain scores in the range $[0,1]$.

%In line with our observations on semantic narrowing as one of the processes leading to semantic variation, we hypothesise that words that exhibit a semantic shift are likely to have higher contextual specificity.
%\raq{so far, there are no observations on semantic narrowing in the qualitative analysis}

%\textbf{contextual specificity}
%\underline{domains} I would expect a positive correlation between this feature and domain shift. Strong collocation can be seen as the step coming before semantic narrowing: a word that in the general language is used in many different contexts, tends to be used only in specific contexts in a domain, and this is highlighted by an high collocation index. The following step is the one in which there is no need to specify the context anymore, and the narrowing process is complete. Example of this scenario are 'yellow' (highly collocated with 'card', but also occuring alone with the narrowed meaning) and ‘window’ ('market window' - 'window').
%
%\underline{communities} I expect the positive correlation for communities. An example is 'theatre' in reddevils: 'theatre of dreams' is the way they call their stadium. This occurs of course very often (strong collocation). But you can find 'theatre' alone as well, with its narrowed meaning of (Manchester) 'stadium'

\paragraph{Dissemination.} Finally, we consider the range of individuals using a given word. A priori, words with the same frequency, prominence, or contextual specificity may differ in their level of social dissemination, i.e., in the proportion of community members using them. We compute a word's dissemination within a community $c$ as follows: 
\begin{eqnarray*}
{\rm Dis}(w,c) & =  & (U^w_c / U_c) \times ({\rm Freq}(w,c) - 1) 
\end{eqnarray*}
where $U^w_c$ is the number of community members who use word $w$ and $U_c$ the total number of members in community $c$. Since words with very high frequencies (such as function words) will be used across the board, we weight the ratio $U^w_c / U_c$ by the inverse of $w$'s frequency.

Word dissemination has been shown to be predictive of changes in word frequency over time \cite{altman-etal:plos-one:2011}. Here we investigate whether it is a determiner of semantic variation. 
%Given our emphasis on social interaction, we expect it to be a key factor: for a shift to affect several domain-related communities, the word must be sufficiently disseminated among them; for a shift to be exclusive of a single sub-community the word can't be highly disseminated if the community shares a substantial number of members with other communities (only if it is isolated from other communities could we expect high dissemination).

%\textbf{dissemination} 
%
%\underline{domains}I expect a positive correlation: if a word undergoes a shift it means that is important in that domain and, in turns, this means that is used by a large number of users.
%
%\underline{communities} I expect positive correlation here as well, for the same reason above. I can also think to an example that I saw in the data: the word 'believer' in LiverpoolFC has high community shift index, and is particularly interesting because until 2016 it was not spread at all; then it was used during a famous interview from the team coach in 2016, and from the moment on it was used by an increasing number of users of the subreddit (i.e. more dissemination). Now that I think about it, probably my hypothesis is somehow biased by the fact that I saw phenomenon of this kind in the data. 
%

\subsection{Results}
\label{sec:factors-results}

\begin{table}\small \centering
\begin{tabular}{@{}l@{\; \  }l@{\; \ }l@{\; \ }l@{\; \ }l@{}}
& ${\rm Freq}$ & ${\rm Pro}$ & ${\rm Spe}$ & ${\rm Dis}$\\\toprule
Programming & 0.96 *** & 0.72 *** & 0.46 *** & 0.37 ***\\
Football& 1.32 *** & 0.81 *** & 0.52 *** & 0.63 *** \\\midrule
%\re{programming} & -- & -- & -- & -- \\
\re{python} & 0.12  & 1.0 \ \  *** & 0.09 \;  &  0.21 ***\\
\re{learn.prog} & 0.02 & 0.63 *** & 0.32 *  & 0.23 **\\\hdashline
%\re{soccer} & -- & -- & -- & -- \\
\re{liverpool} & 0.26  ** & 0.47 ** & 0.18  & 0.38 *** \\
\re{red.devils} & 0.16 &  0.42 ** & 0.16  & 0.20 *  \\\bottomrule
\end{tabular}
\caption{Effect size (Cohen's $d$) and unpaired two-sample $t$-test significance level (***$p\!<\!.001$, **$p\!<\!.01$, *$p\!<\!.05$) for each feature.}\label{tab:factors}
\end{table}

To investigate the role of the features introduced above, we test whether their values are significantly different in words that exhibit a strong semantic shift (words with  {\bf dsi} / {\bf csi} values equal or larger than 2 standard deviations above the mean within a domain or community) and words with no semantic variation (with index values lower than one standard deviation above the mean).

%according to our indices and words that do not. We extend the approach of Section~\ref{sec:eval}: instead of taking only the 10 top and bottom words in the positive range of {\bf dsi} / {\bf csi}, we consider all words with {\bf dsi} / {\bf csi} values above 2 standard deviations above the mean to exhibit a strong semantic shift, and those words whose indices are lower than one standard deviation above the mean to exhibit no shift. 

At the domain level, we find very robust patterns for all features: the words that have undergone a strong domain shift have significantly higher frequency, prominence, contextual specificity, and social dissemination  in the two domains considered, Programming and Football. Table~\ref{tab:factors} shows the significance level of a unpaired two-sample $t$-test and the effect size for each feature.

At the community level, since the shifts for the \re{programming} and \re{soccer} communities were not validated in our extrinsic evaluation (Section~\ref{sec:lm-results}), we do not consider these communities here. For the other 4 communities, we find a systematic pattern: words that exhibit a semantic shift particular to a community are significantly {\em more} prominent in that community than in other domain-related communities, and {\em less} disseminated within that community than words that do not exhibit a shift. The significance of frequency and specificity vary per community. A summary is given in Table~\ref{tab:factors}.

\subsection{Qualitative Analysis}
\label{sec:factors-analysis}

Prominence (Pro) is significantly related to meaning shift in both domains and communities. For example, the word `box' has high \textbf{dsi} and Pro=0.69 in Football, whereas in Programming has low \textbf{dsi} and Pro=0.5. The same is true for communities: `believers' has high \textbf{csi} in \re{liverpool} and Pro=0.73, while in the other two Football communities has low \textbf{csi} and Pro values below 0.2.
Moreover, as expected (see \ref{sec:factors-features}), common words that undergo a meaning shift tend to have high values of Prominence, but still lower than those of jargon and slang words, which have values close or equal to 1, like `hat-trick' (Pro=1 in Football) and `bitwise' (Pro=1 in Programming).

For the other features considered we found a positive correlation only with meaning change at domain level. Our intuition is that this reflects an inherent difference between domain and community shift, which can be explained referring to the process of linguistic innovation described by \newcite{milroy1985linguistic}. Innovations - which in our case are meaning shifts - originate in a community and are initially adopted by a circumscribed number of people. This explains why \textbf{csi} is not related to high frequency and correlates with low values of dissemination. Some innovations then spread in the community and possibly in other communities in the domain. At this point, the innovation is widely accepted and used by the majority of speakers. This is the kind of shift captured by \textit{dsi}, which therefore correlates positively with Frequency and Dissemination. Finally, Specificity is based on the collocational score of a word. The positive correlation between frequency of a word and its possibility to occur in collocations have been pointed out in different studies (e.g. \newcite{shin2008beyond}). Thus, it is not surprisingly that only high \textbf{dsi} words, that are highly frequent, correlate positively also with Specificity, while this does not happen with \textbf{csi} words, which have in general low frequency.

Concluding, we note how the syntactic crystallization captured by Specificity can be considered as a part of the wider process \textit{narrowing} of meaning to which some words undergo. For example, the word `yellow' occurs in many different contexts in the general language, while it is used mostly in the collocation `yellow card' in  Football. The strength of the collocation is such that at some point speakers do not need to specify `card' anymore, and `yellow' narrows down its meaning to that of the collocation. The result of this process is the use of the word in sentences like `Terry got a very stupid \textit{yellow}'.


%Finally, we note how words with high \textbf{dsi} tend to occur often in fixed syntactic structures: `yellow', for example, occurs most of the time in the collocation `yellow card'. We see tihs process as part of  


%structures, eg: ‘win [the/a/many] title’, ’transfer window’, ‘in the box/outside the box’, ‘yellow card'. From my point of view, this aspect reflects the narrowing process we were discussing some weeks ago, whereby a word that in the general language is used in many different contexts, tends to be used only in specific contexts in a domain. Somehow, it is like if the collocation was the step before the ‘full’ meaning shift, i.e.: ‘yellow card’ occurs so often that, at some point, the speakers do not need to specify ‘card’ anymore, and ‘yellow’ changes its meaning, including the whole collocation (remember the example: "Terry got a ver stupid yellow”).

%I am looking also to the programming domain, and somehow the effect here is less clear: for example, ‘queries’ indeed occurs very often with sql/ql, but also in other different structures. However, for words like ‘scope’, ’network’, ‘learn' I don’t see this effect. I need to investigate more this thing.

%Finally, probably the same reasoning could go also for community meaning shift. Let’s consider the case of ‘92’: for Reddevils fans, it often goes in phrases like ’the class of 92’, while its usage is much more varied within the other soccer communities.




%The other features seem to indicate a substantial difference between domain and community shift, i.e.: while domain shift is observed when the new meaning of a word is already established and widespread across communities, at community level the shift is marked by novelty and by the fact of being circumscribed. This is in line with the idea that linguistic innovation orginates in the interaction between singles speakers in a community, before spreading in that community and in the others of the same domain \newcite{milroy1985linguistic}. 

%Adopting this perspective, it is possible to see why domain shift positively correlates with high frequency and diffusion among users. Additionally, high Specialization indicates a certain degree of crystallization of the linguistic structure in which a word occurs, possibly as a consequence of its frequent usage. 
%At the opposite, novelty of shift at the community level is mirrored by the fact that the new meaning is adopted by a limited number of users and, accordingly, that is not very frequent in the community overall. 


%
%\begin{table*}[ht]
%\begin{small}
%\begin{tabular*}{\columnwidth}{lcc|cc|cc|cc}
%
% \bf domain  & \multicolumn{2}{c|}{\bf Freq} & \multicolumn{2}{c}{\bf Prom}& \multicolumn{2}{c|}{\bf Spec} & \multicolumn{2}{c|}{\bf Diss}\\
%  & \bf p value & \bf cohesion &  \bf p value  & \bf cohesion &  \bf p value  & \bf cohesion &  \bf p value  & \bf cohesion \\
%
%Programming & - & 0.958 & -  & 0.717 & - & 0.4597 & - & 0.374 \\
%Soccer & -  & 1.318 & - & .801 & - &0.524 & - & 0.632 \\
%\end{tabular*}
%\caption{...}\label{tab:factors_domain}
%\end{small}
%\end{table*}
%
%
%
%\begin{table*}[ht]
%\begin{small}
%\begin{tabular*}{\columnwidth}{lcc|cc|cc|cc}
%
% \bf domain  & \multicolumn{2}{c|}{\bf Freq} & \multicolumn{2}{c}{\bf Prom}& \multicolumn{2}{c|}{\bf Spec} & \multicolumn{2}{c|}{\bf Diss}\\
%  & \bf p value & \bf cohesion &  \bf p value  & \bf cohesion &  \bf p value  & \bf cohesion &  \bf p value  & \bf cohesion \\
%
% \re{python} & 0.306  & 0.123 & - & 1.033 & 0.314 & 0.086 & - & 0.2049\\
% \re{learn.prog} & 0.824 & 0.025 & - & 0.629 & 0.04 & 0.319 & - & 0.229\\\hdashline
% \re{liverpool} & - & 0.265 & - & 0.475 & 0.205 & 0.179 & - & 0.383\\
% \re{red.devils} & 0.120  & 0.160 &  - & 0.424 & 0.236 & 0.158 & - & 0.201 \\
%\end{tabular*}
%\caption{...}\label{tab:factors_community}
%\end{small}
%\end{table*}

==> measures.tex <==
\section{Temporary section to define notation and measures}

Let $C$ be a set of {\em communities of practice} and let $\star$ denote the {\em general community}, reflecting general language use across all communities. We use subsets such as $D\subset C$ to denote sets of communities related by a certain \emph{domain}.

In our setting, the language use of a community $c \in C$ is modelled by the interactions about a given theme among a set of individuals over a certain period of time. More concretely, we leverage data from Reddit discussion forums to model communities of practice. For example, the set of users affiliated with the sub-reddit {\em Liverpool} constitutes a community, and we take all posts and comments by these users within that sub-reddit over a given time span to represent the linguistic practices of such a community. In addition, the {\em Liverpool} and {\em Chelsea} communities are both concerned with the common domain of football. Finally, to capture the linguistic practices of the general community $\star$, we consider a sample of exchanges within {\em all} sub-reddits over a given period of time as a proxy for general language use. 
 
Now, assume we have created  word embeddings $w_c$, $w_\star$ for each word $w$ encoding how $w$ is used within each community $c \in C$ and in the general language $\star$, respectively. 
 
For any two vectors $v,v'\in\mathbb{R}^k$, let $\csim(v,v')$ denote their \emph{cosine similarity}. Given two sets of communities $A,B\subseteq C\cup\{\GenCom\}$, we use $\Sim^w_{A,B}$ to refer to the following multiset of similarity values\footnote{Recall that, unlike a set, a multiset allows multiple instances of the same elements. This is appropriate in our case since cosine similarity values for different pairs of words may be identical.} for word $w$:\footnote{In practice, in case $A=B$, we only compute one cosine similarity value for every unordered pair rather than for every ordered pair. Observe that this does not affect either the mean or the standard deviation of the multiset.} 
\[\begin{array}{r@{\ }c@{\ }r}
\Sim^w_{A,B} & = & \{ \csim(w_a,w_b) \mid (a,b)\in A\times B\ \ \ \ \\ 
	&& \text{with}\ a\not=b\}
\end{array}\]
 
\noindent
Let $S$ and $S'$ be two such multisets of similarity values. To measure the extent to which these values are higher in $S$ than in $S'$, we use the following index, where $\mu$ and $\sigma$ are the mean and the standard deviation, respectively:
\begin{eqnarray*}
\Index(S,S') & = & [\mu(S)-\sigma(S)] - [\mu(S')+\sigma(S')]
\end{eqnarray*}

\noindent 
The intuition behind this general formulation should be clear: we expect the similarity values in $S$ to be higher than those in $S'$
We can now use this generic index to construct several specific indices to quantify different types of semantic shifts.

%==== dsi =======
 \paragraph{Domain-specific semantic shift:} We consider that a word $w$ exhibits a domain-specific semantic shift if its meaning is relatively constant across communities with a common domain, while being distinct from its use in general language. The \emph{domain shift index} ${\bf dsi}^w(D)$ captures exactly this, for a given domain $D\subset C$ and word~$w$:
\begin{eqnarray*}
{\bf dsi}^w(D) & = & \Index(\Sim^w_{D,D},\Sim^w_{D,\{\GenCom\}})
\end{eqnarray*}

\noindent
The higher the {\em domain shift index} of a word, the more pronounced its semantic shift within a domain with respect to the general language.

\raq{To calculate ${\bf dsi}^w(D)$, the min cardinality of $D$ is 2. If $|D| = 2$, then $\mu(\Sim^w_{D,D}) = \csim(w_{c_1}, w_{c_2})$ and $\sigma(\Sim^w_{D,D}) = 0$}
 
% ==== csi ====
  \paragraph{Community-specific semantic shift:} We now want to quantify the degree to which a given word $w$ exhibits a semantic shift particular to a community $c$. We can consider two types of shifts concerned with (i) how distant $w$'s use in $c$ is from its use in other domain-related communities and (ii) how distant it is from its use in the general language compared to other domain-related communities. Although compatible, these two possible community-specific shifts do not need to be connected. We thus quantify them independently by means of two different indices. 
  
The {\em community shift index} ${\bf csi}^w(c,D)$ of community $c$ relative to domain $D\subset C$, with $c\in D$, for word~$w$ is defined as follows, where $D\setminus\{c\}$ denotes the set of communities in domain $D$ except for $c$: 
\begin{eqnarray*}
{\bf csi}^w(c,D) & = & \Index(\Sim^w_{D\setminus\{c\},D\setminus\{c\}},\Sim^w_{\{c\},D\setminus\{c\}})
\end{eqnarray*}
 
\noindent 
The index measures the extent to which the meaning of $w$ in $c$ differs from its common meaning among other communities in domain $D$. The higher the ${\bf csi}^w(c,D)$ for word $w$, the more pronounced the difference between the use of $w$ in $c$ and in other communities concerned with the same domain.

We now define the second type of {\em community shift index}, ${\bf csi}_{\star}^w(c,D)$ of community $c$ relative to the general language $\star$ and domain $D\subseteq C$, with $c\in D$, for word~$w$:
\begin{eqnarray*}
{\bf csi}_{\star}^w(c,D) & = & \Index(\Sim^w_{D\setminus\{c\},\{\GenCom\}},\Sim^w_{\{c\},\{\GenCom\}})
\end{eqnarray*}

%The {\em community shift index} of community $c$ relative to some subset  $C'\subseteq C$, with $c\in C'$, for word~$w$ measures the extent to which the meaning of $w$ in $c$ is more dissimilar from the general language than its meaning in other communities (which may or may not belong to the same domain as $c$). 
%  \begin{eqnarray*}
%{\bf \star csi}^w(c,C') & = & \Index(\Sim^w_{C'\setminus\{c\},\{\GenCom\}},\Sim^w_{\{c\},\{\GenCom\}})
%\end{eqnarray*}

\noindent
This index measures the extent to which the meaning of $w$ in $c$ is more dissimilar from the general language than the meaning of $w$ in other communities belonging to domain $D$. Again, the higher the ${\bf csi}_{\star}^w(c,D)$ for word $w$, the stronger the shift. 
  
\raq{To calculate ${\bf csi}^w(c,D)$ and ${\bf \star csi}^w(c,D)$, the min cardinality of $D$ and $C'$ is 3.}

 

==> model.tex <==
\section{marco}

We adapt the geoSGML model introduced by \newcite{bamman-dyer-smith:2014} for geo-located language to communities of practice.
The model is an extension of the SkipGram model by \newcite{mikolov2013efficient}. In the original SkipGram model each input word is represented by a single real-valued vector (the hidden layer $h$ of the model) which encodes all the occurrences of a word in the corpus. The same kind of representation is created also in the geoSGML model, where it is defined $h_{\it Main}$. In addition to $h_{\it Main}$, $n$ vector representations for the same word are computed, where $n$ is the number of variables to be considered. In our case, $n$ corresponds to the size of the set of communities $C=\{{\it LiverpoolFC, Reddevils,} \ldots\}$. For a target word $w$, the parameters of $h^w_{Main}$ are updated for any occurrence of $w$, while the parameters of $h^w_{Ci}$ are updated only when the the target word is observed in the corpus representing the language of  community $i$. The model therefore learns several embeddings for the same word form: one general embedding and $|C|$ \textit{deviation vectors} \newcite{kulkarni2016freshman}, one for each community. The final vector representation of target word $w$ in community $i$ is given by the sum of the $Main$ and the $Ci$ deviation vectors: $h^w_{Main} + h^w_{Ci}$. 

For the purposes of our investigation, we want to obtain, for a target word $w$, (i) a representation of its meaning in each of the communities of practice we considered; (ii) a more general meaning representation of the word at the level of the Reddit community, which we consider as the general meaning of the word. If our set of variables $C$ included samples of language from \textit{all} the existing subreddits, the vector $h_{\it Main}$ would represent the general meaning of words as defined in (ii). However, our set of variables $C$ only includes few subreddits. Therefore, in order to obtain a representation of the general meaning of the word in Reddit, we add to the set $C$ another variable that we call $General Language$ and whose corpus is created by randomly extracting samples of language from Reddit. As for the other communities, the model learns for each word a deviation vector $h^w_{C\_General\_Lanaguage}$ which is then summed up with the $Main$ vector in order to obtain the word representation in Reddit general language.


==> qualitative_analysis.tex <==
\section{marco}

\textbf{domains}


We manually inspected the corpora in order to qualitatively evaluate the results obtained with.





git pull
At the domain level, the shift of meaning for the words with high \textbf{dsi} values is clear, both for $Programming$ and the $Football$. As an example, let's consider the word 'cross' in the soccer domain, whose domain index shift value is [normalized score?]: while in the general language the term is used to refer to the action of traversing or going across a space, in the soccer community it refers almost exclusively to a kind of pass usually directed from outside the penalty area to inside it, as in the  example: 'Take the ball, cross towards the striker'. The difference in usage clearly emerges by looking at closest neighbours of the term in the $Football$ domain and in the general language reported in table [n]: while in the general language the closest words are object or spaces that are usually crossed ('bridge', 'mountain', 'street'), in the soccer domain the most related words are similar actions ('pass', 'shot'), actions that usually follow a cross ('header'), and the place where the cross usually comes from or is directed to ('byline', 'box', 'corner'). At the opposite, words with low values of domain index shift are used in the soccer domain in contexts that are largely similar to the ones in which they occur in general language. This is the case, for example, of the term 'computer', which does not undergo any kind of shift within the soccer domain (domain index shift value is=[normalized score?]). The list of closest neighbours (table n) confirms that there is no meaning shift, as the most similar words for 'computer' are almost the same both for the soccer community and the general language. 
For the programming domain we observe the same kind of correlation between the values of domain shift index and differences in usage. For example, the high index value of the term 'commit' (insert value) reflects the fact that in the programming domain the term denotes a specific action usually performed with version control system, while in the general language it refers to a completely different action, and occurs in contexts like 'commit an homicide'. At the opposite, the term 'decade' (insert value), is used similarly in general language and programming domain, where it does not undergo any kind of meaning shift. Also in this case, differences in meaning shift are mirrored in the list of closets neighbours: while there is no common neighbour for 'commit' in programming domain and general language, there is a large overlap for 'decade' in the two lists.  
Finally, we note that while few words undergo meaning shift due to the domain ('cross', 'commit'), the large majority of words do not change their meaning in different communities. Consequently, we would expect for these words a common meaning in the different communities and in general language. This what we find when we look at the usage and the nearest neighbours of words with low domani meaning shift values, e.g. car, whose meaning is stable across communities and in general language. 

\mdt{should we add that different communities in the same domain have similar lists of closest neighbours for words with high domain index shift value?}
